Illuminating English Letters Using a Flying Light Speck

This paper presents the design and implementation of a Flying Light Speck (FLS) to illuminate English letters. The FLS uses its onboard camera and computing to localize and follow a trajectory to illuminate a letter. We evaluate the illuminations quantitatively and qualitatively. The latter is based on an IRB approved human subject study with 20 participants. The obtained results show a 42 to 56 millimeter error that impacts the detection of letters. A key finding is that the order in which the illumination of letters is presented to subjects has a significant effect on detection duration.

==> letters.tex <==
% Terminology

% Problem statement 1: illuminate english letters using an FLS
% time to illuminate a letter based on FLS speed and acceleration of an FLS
% How is the trajectory sent to the FLS?
% Problem statement 2: compute a trajectory for english letters
% Converting sparse points to an interpolated smooth writing path
% How is the writing path converted to the trajectory based on the speed and accel?

To illuminate a letter using an FLS, a human authors several points in a 2D coordinate system that describes a letter, see the red points in Figure~\ref{fig:trajectory}.

A program computes one or more segments 

To illuminate a letter using an FLS, we 1) design a writing path for a letter and 2) convert the writing path to a trajectory.
The former means a human authors several points in a 2D coordinate system that describes a letter, see the red points in Figure~\ref{fig:trajectory}.
The latter is computed using a piece of software, see Figure~\ref{NEW FIGURE}.
The resulting trajectories may be visualized using Blender.
Alternatively, the FLS uses its localization technique to travel along the trajectory and illuminate the letter.
We use both in the evaluation section of this paper.

The {\em Writing Path} is defined as a sequence of 3D continuous lines or curves.
One may author different writing paths for a letter. 
However, one must select one writing path to illuminate the letter.
%There is one writing path for a letter. 
%The FLS executes the trajectory. 
The {\em Writing Path} is defined as a sequence of 3D continuous lines or curves to draw a letter. 
%The {\em Writing Path} is defined as the 3D path traveled by the FLS. 
More formally, it consists of a sequence of one or more human authored segments. 
A segment may be a straight line or a curve, e.g., an arc, oval, etc. 
A {\em Segment} is a continuous portion of the Writing Path defined by a series of human authored points.
It has a start point, an end point, and optionally, a set of intermediate points that describe its shape. 
The discrete points of a segment are converted into a smooth, continuous path.
We use B-splines for this purpose.

Each segment is designated as either {\em lit} or {\em dark}.
The FLS illuminates its LED when traversing a lit segment, analogous to a pen stroke, where the tip is on the paper. On the other hand, the FLS turns its LED off when traversing a dark segment. This is used for repositioning to the start of a lit segment.  It is analogous to lifting the pen from the paper to move to a new location. To enable the FLS to write the letter repeatedly, we define a {\em Looping Writing Path}, which is a modified Writing Path designed to be played as a continuous animation loop.
To form the loop based on a Writing Path, if the start and end points of a Writing Path are not the same, a final Dark Segment is added. We call it the {\em Return Segment}. It connects the end point of the last segment to the start point of the first segment, creating a closed, endlessly repeatable path. Table \ref{tab:segments} presents the number of each segment type for the different English letters.

\begin{table}[]
    \centering
    \caption{The number of Segments for Writing Paths of English letters}

    \begin{tabular}{c|c|c|c|c}
    \hline
         Letter	& \# Lit & \# Dark & \# Return & Total\\
     \hline
        A & 3 & 1 & 1 & 5  \\
        B & 3 & 0 & 0 & 3  \\
        C & 1 & 0 & 1 & 2  \\
        D & 2 & 0 & 0 & 2  \\
        E & 4 & 1 & 1 & 6  \\
        F & 3 & 1 & 1 & 5  \\
        G & 3 & 0 & 1 & 4  \\
        H & 3 & 2 & 1 & 6  \\
        I & 3 & 2 & 1 & 6  \\
        J & 2 & 1 & 1 & 4  \\
        K & 3 & 1 & 1 & 5  \\
        L & 2 & 0 & 1 & 3  \\
        M & 4 & 0 & 1 & 5  \\
        N & 3 & 0 & 1 & 4  \\
        O & 1 & 0 & 0 & 1  \\
        P & 2 & 0 & 1 & 3  \\
        Q & 2 & 1 & 1 & 4  \\
        R & 3 & 1 & 1 & 5  \\
        S & 1 & 0 & 1 & 2  \\
        T & 2 & 1 & 1 & 4  \\
        U & 2 & 0 & 1 & 3  \\
        V & 2 & 0 & 1 & 3  \\
        W & 4 & 0 & 1 & 5  \\
        X & 2 & 1 & 1 & 4  \\
        Y & 3 & 1 & 1 & 5  \\
        Z & 3 & 0 & 1 & 4  \\
     \hline
    \end{tabular}
    \label{tab:segments}
\end{table}

The trajectory is the time-based flight plan generated from the Writing Path. It is a discrete sequence of setpoints that dictates FLS’s state over time. A trajectory consists of a series of setpoints, which are sampled from the continuous Writing Path at a rate determined by the animation’s frame rate. Each setpoint is a single instruction in the trajectory that defines the desired FLS position and velocity at a specific point in time. 
The FLS follows the trajectory from the start point to the end point over a set duration.
The acceleration and the maximum speed of the FLS are used to compute the Trajectory. The setpoints are computed for each segment, then combined to create the full trajectory. The time step between subsequent setpoints is fixed, $\frac{1}{frame~rate}$. We use kinematics to compute the distance traveled at the fixed time steps, considering acceleration, cruising with max speed, and deceleration. 
We map the distances to a point on the segment. The time to illuminate a letter depends on the length of each segment, FLS max speed, and FLS acceleration.

The trajectories for Letter E and N in this study were generated with a max speed of $0.75 m/s$ and an acceleration of $0.1 m/s^2$. 
For letters S and O, a constant speed of $0.25 m/s$ was used without acceleration and deceleration.
Figure \ref{fig:trajectory} presents a visualization of these trajectories for Letters O, S, N, and R.

\begin{figure*}
    \centering
    \includegraphics[width=0.2\linewidth]{figs/O_0.4x0.6m_fps30_speed0.25.png}
    ~\includegraphics[width=0.18\linewidth]{figs/S_0.4x0.6m_fps30_speed0.25.png}
    ~\includegraphics[width=0.2\linewidth]{figs/N_0.4x0.6m_fps30_speed0.75_accel0.1.png}
    ~\includegraphics[width=0.2\linewidth]{figs/E_2_0.4x0.6m_fps30_speed0.75_accel0.1.png}
    \caption{Computed trajectory based on the Writing Path. The red line shows the un-interpolated points of the segments. Yellow shows the trajectory for the Lit Segment, Gray is for the Dark Segment, and Blue is the Return Segment. }
    \label{fig:trajectory}
\end{figure*}
